CARS: the CFHTLS-Archive-Research Survey; I. Five-band multi-colour data from 37 sq. deg. CFHTLS-Wide observations

We present the CFHTLS-Archive-Research Survey (CARS). It is a virtual multi-colour survey based on public archive images from the CFHT-Legacy-Survey. Our main scientific interests in CARS are optical searches for galaxy clusters from low to high redshift and their subsequent study with photometric and weak-gravitational lensing techniques. As a first step of the project we present multi-colour catalogues from 37 sq. degrees of the CFHTLS-Wide component. Our aims are to create astrometrically and photometrically well calibrated co-added images. Second goal are five-band (u*, g', r', i', z') multi-band catalogues with an emphasis on reliable estimates for object colours. These are subsequently used for photometric redshift estimates. The article explains in detail data processing, multi-colour catalogue creation and photometric redshift estimation. Furthermore we apply a novel technique, based on studies of the angular galaxy cross-correlation function, to quantify the reliability of photo-z's. The accuracy of our high-confidence photo-z sample (10-15 galaxies per sq. arcmin) is estimated to $\sigma_{\Delta_z/(1+z)}\approx 0.04-0.05$ up to i'<24 with typically only 1-3% outliers. Interested users can obtain access to our data by request to the authors.

==> table.tex <==
\begin{longtable}{llrrrrrrp{2.5cm}}
\caption{\label{tab:CARSquality}\CARS data quality overview: 
The first column lists: \CARS field-naming convention; CFHTLS
field-naming convention; effective field area after image masking. 
The seventh
column contains magnitude comparisons of \CARS fields with those
from TERAPIX \Tthree (indicated by \textbf{(T)}) and \MegaPipe
(indicated by \textbf{(M)}). Magnitude offsets are always given as
$m_{\rm CARS}-m_{\rm other}$. See the text for more details.} \\
\hline\hline
\multicolumn{1}{c}{Field/Area} & \multicolumn{1}{c}{Filter} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{expos. time} & \multicolumn{1}{c}{$m_{\rm lim}$} & \multicolumn{1}{c}{Sloan} & \multicolumn{1}{c}{T3/MegaP.} & \multicolumn{1}{c}{seeing} & \multicolumn{1}{c}{comments} \\
\multicolumn{1}{c}{[sq. deg.]} & & & \multicolumn{1}{c}{[s]} & \multicolumn{1}{c}{[AB mag]} & \multicolumn{1}{c}{$\Delta m \times 100$} & \multicolumn{1}{c}{$\Delta m \times 100$} & \multicolumn{1}{c}{[$''$]} & \\
\hline
\endfirsthead
\hline\hline
\multicolumn{1}{c}{Field/Area} & \multicolumn{1}{c}{Filter} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{expos. time} & \multicolumn{1}{c}{$m_{\rm lim}$} & \multicolumn{1}{c}{Sloan} & \multicolumn{1}{c}{T3/MegaP.} & \multicolumn{1}{c}{seeing} & \multicolumn{1}{c}{comments} \\
\multicolumn{1}{c}{[sq. deg.]} & & & \multicolumn{1}{c}{[s]} & \multicolumn{1}{c}{[AB mag]} & \multicolumn{1}{c}{$\Delta m \times 100$} & \multicolumn{1}{c}{$\Delta m \times 100$} & \multicolumn{1}{c}{[$''$]} & \\
\hline
\endhead
\hline
\endfoot
%
\texttt{W1m0p1} & u* & 5 & 3000.51 & 25.27 & - & $0.0 \pm 0.8$ \textbf{(T)}& 1.00 &  \\
\texttt{[w1.$-$0$+$1]} & & & & & & $-0.4 \pm 1.3$ \textbf{(M)} & & \\
(0.84) & g' & 5 & 2500.45 & 25.55 & - & $-0.4 \pm 0.5$ \textbf{(T)}& 0.90 &  \\
 & & & & & & $-7.1 \pm 0.9$ \textbf{(M)} & & \\
 & r' & 3 & 1500.28 & 24.72 & - & $-1.9 \pm 1.0$ \textbf{(T)}& 0.79 &  \\
 & i' & 7 & 4305.67 & 24.61 & - & $-0.1 \pm 0.8$ \textbf{(T)}& 0.85 &  \\
 & & & & & & $-0.8 \pm 0.7$ \textbf{(M)} & & \\
 & z' & 11 & 6601.19 & 23.88 & - & $0.2 \pm 1.5$ \textbf{(T)}& 0.79 &  \\
 & & & & & & $-7.7 \pm 1.1$ \textbf{(M)} & & \\
\hline
\texttt{W1m0p2} & u* & 5 & 3000.58 & 25.35 & - & $-0.6 \pm 1.1$ \textbf{(T)}& 1.00 &  \\
\texttt{[w1.$-$0$+$2]} & & & & & & $-2.2 \pm 1.5$ \textbf{(M)} & & \\
(0.76) & g' & 7 & 3500.46 & 25.72 & - & $-0.5 \pm 1.0$ \textbf{(T)}& 0.95 &  \\
 & & & & & & $-2.5 \pm 0.9$ \textbf{(M)} & & \\
 & r' & 2 & 1000.18 & 24.61 & - & $-0.5 \pm 0.5$ \textbf{(T)}& 0.82 & no ch. 21, 35 \\
 & i' & 7 & 4305.66 & 24.72 & - & $1.3 \pm 2.4$ \textbf{(T)}& 0.74 &  \\
 & & & & & & $0.2 \pm 1.8$ \textbf{(M)} & & \\
 & z' & 10 & 6000.83 & 23.64 & - & $-1.2 \pm 3.5$ \textbf{(T)}& 0.79 & fr. res. \\
 & & & & & & $-7.3 \pm 1.5$ \textbf{(M)} & & \\
\hline
\texttt{W1m0p3} & u* & 5 & 3000.58 & 25.27 & - & $-1.0 \pm 1.4$ \textbf{(T)}& 0.87 &  \\
\texttt{[w1.$-$0$+$3]} & & & & & & $5.3 \pm 1.2$ \textbf{(M)} & & \\
(0.75) & g' & 5 & 2500.49 & 25.56 & - & $-0.7 \pm 0.8$ \textbf{(T)}& 0.90 &  \\
 & & & & & & $-1.9 \pm 0.6$ \textbf{(M)} & & \\
 & r' & 2 & 1000.18 & 24.62 & - & $-1.2 \pm 0.5$ \textbf{(T)}& 0.85 & no ch. 21, 35 \\
 & i' & 7 & 4305.65 & 24.59 & - & $-0.5 \pm 0.7$ \textbf{(T)}& 0.74 &  \\
 & & & & & & $-0.8 \pm 0.5$ \textbf{(M)} & & \\
 & z' & 10 & 6000.84 & 23.59 & - & $-1.3 \pm 2.7$ \textbf{(T)}& 0.82 & fr. res. \\
 & & & & & & $-8.1 \pm 1.4$ \textbf{(M)} & & \\
\hline
\texttt{W1m1p1} & u* & 7 & 4200.60 & 25.50 & - & - & 1.00 &  \\
\texttt{[w1.$-$1$+$1]} & g' & 8 & 4000.76 & 25.73 & - & - & 0.66 &  \\
(0.84) & r' & 2 & 1000.20 & 24.51 & - & - & 0.59 &  \\
 & i' & 9 & 5535.73 & 24.53 & - & - & 0.79 &  \\
 & z' & 6 & 3600.40 & 23.30 & - & - & 0.75 &  \\
\hline
\texttt{W1m1p2} & u* & 5 & 3000.52 & 25.03 & - & $-12.0 \pm 0.6$ \textbf{(T)}& 0.92 &  \\
\texttt{[w1.$-$1$+$2]} & & & & & & $-9.2 \pm 1.5$ \textbf{(M)} & & \\
(0.82) & g' & 5 & 2500.48 & 25.44 & - & $3.3 \pm 0.7$ \textbf{(T)}& 0.87 &  \\
 & & & & & & $-4.1 \pm 1.0$ \textbf{(M)} & & \\
 & r' & 4 & 2000.38 & 24.80 & - & $1.0 \pm 2.2$ \textbf{(T)}& 0.87 &  \\
 & & & & & & $-2.1 \pm 2.0$ \textbf{(M)} & & \\
 & i' & 7 & 4305.66 & 24.52 & - & $-0.1 \pm 1.8$ \textbf{(T)}& 0.71 &  \\
 & & & & & & $1.6 \pm 2.1$ \textbf{(M)} & & \\
 & z' & 11 & 6601.18 & 23.87 & - & $-1.1 \pm 1.5$ \textbf{(T)}& 0.71 & fr. res. \\
 & & & & & & $0.3 \pm 0.8$ \textbf{(M)} & & \\
\hline
\texttt{W1m1p3} & u* & 5 & 3000.50 & 24.95 & - & $-18.3 \pm 0.5$ \textbf{(T)}& 0.79 &  \\
\texttt{[w1.$-$1$+$3]} & g' & 3 & 1500.30 & 25.22 & - & $1.0 \pm 0.8$ \textbf{(T)}& 0.77 &  \\
(0.76) & r' & 2 & 1000.23 & 24.58 & - & $1.4 \pm 0.8$ \textbf{(T)}& 0.79 & no ch. 21, 35 \\
 & i' & 7 & 4305.70 & 24.58 & - & $-0.3 \pm 1.0$ \textbf{(T)}& 0.74 &  \\
 & z' & 10 & 6001.00 & 23.43 & - & $-11.9 \pm 2.3$ \textbf{(T)}& 0.71 & fr. res. \\
\hline
\texttt{W1p1m1} & u* & 5 & 3000.42 & 25.26 & $12.2 \pm 5.5$ & - & 0.85 &  \\
\texttt{[w1.$+$1$-$1]} & g' & 6 & 3000.47 & 25.79 & $2.7 \pm 2.8$ & - & 0.87 &  \\
(0.85) & r' & 2 & 1000.16 & 24.50 & $4.2 \pm 3.4$ & - & 0.71 &  \\
 & i' & 7 & 4305.53 & 24.85 & $5.2 \pm 4.8$ & - & 0.71 &  \\
 & z' & 6 & 3600.40 & 23.52 & $1.3 \pm 5.7$ & - & 0.85 &  \\
\hline
\texttt{W1p1p1} & u* & 5 & 3000.47 & 25.28 & - & $0.6 \pm 0.9$ \textbf{(T)}& 0.92 &  \\
\texttt{[w1.$+$1$+$1]} & & & & & & $6.6 \pm 0.7$ \textbf{(M)} & & \\
(0.75) & g' & 10 & 5000.88 & 25.97 & - & $-0.3 \pm 0.7$ \textbf{(T)}& 0.95 &  \\
 & & & & & & $-2.0 \pm 0.5$ \textbf{(M)} & & \\
 & r' & 2 & 1000.18 & 24.57 & - & $-1.6 \pm 0.6$ \textbf{(T)}& 0.85 &  \\
 & i' & 7 & 4305.72 & 24.70 & - & $-0.1 \pm 0.8$ \textbf{(T)}& 0.82 &  \\
 & & & & & & $-0.5 \pm 0.5$ \textbf{(M)} & & \\
 & z' & 12 & 7201.21 & 23.94 & - & $0.9 \pm 1.5$ \textbf{(T)}& 0.74 & fr. res. \\
 & & & & & & $-9.3 \pm 1.3$ \textbf{(M)} & & \\
\hline
\texttt{W1p1p2} & u* & 5 & 3000.48 & 25.29 & - & $-3.9 \pm 1.0$ \textbf{(T)}& 1.00 &  \\
\texttt{[w1.$+$1$+$2]} & g' & 5 & 2500.42 & 25.60 & - & $-1.3 \pm 1.0$ \textbf{(T)}& 0.87 &  \\
(0.83) & r' & 2 & 1000.16 & 24.50 & - & $-0.1 \pm 0.6$ \textbf{(T)}& 0.74 &  \\
 & i' & 6 & 3690.57 & 24.45 & - & $-0.1 \pm 1.0$ \textbf{(T)}& 0.77 &  \\
 & z' & 10 & 6001.00 & 23.60 & - & $-0.4 \pm 1.8$ \textbf{(T)}& 0.63 & fr. res. \\
\hline
\texttt{W1p1p3} & u* & 5 & 3000.47 & 25.30 & - & $-2.7 \pm 1.1$ \textbf{(T)}& 0.95 & no ch. 21, 35 \\
\texttt{[w1.$+$1$+$3]} & & & & & & $-1.8 \pm 1.7$ \textbf{(M)} & & \\
(0.80) & g' & 5 & 2500.42 & 25.53 & - & $2.4 \pm 0.8$ \textbf{(T)}& 0.95 & no ch. 21, 35 \\
 & r' & 4 & 2000.22 & 24.72 & - & $-1.4 \pm 1.4$ \textbf{(T)}& 0.89 & no ch. 21, 35 \\
 & i' & 8 & 4920.84 & 24.63 & - & $-0.4 \pm 0.8$ \textbf{(T)}& 0.95 & no ch. 21, 35 \\
 & z' & 10 & 6001.03 & 23.63 & - & $-0.9 \pm 2.2$ \textbf{(T)}& 0.69 & no ch. 21, 35; fr. res. \\
 & & & & & & $-9.9 \pm 1.7$ \textbf{(M)} & & \\
\hline
\texttt{W1p2p1} & u* & 5 & 3000.53 & 25.32 & - & $-3.1 \pm 1.4$ \textbf{(T)}& 1.00 & no ch. 31 \\
\texttt{[w1.$+$2$+$1]} & g' & 5 & 2500.45 & 25.56 & - & $-1.9 \pm 1.1$ \textbf{(T)}& 1.00 & no ch. 31 \\
(0.84) & r' & 2 & 1000.18 & 24.42 & - & $-2.8 \pm 0.6$ \textbf{(T)}& 0.95 & no ch. 31 \\
 & i' & 8 & 4960.74 & 24.63 & - & $0.6 \pm 0.6$ \textbf{(T)}& 0.90 & no ch. 31 \\
 & z' & 10 & 6000.82 & 23.74 & - & $-0.9 \pm 2.2$ \textbf{(T)}& 0.71 & no ch. 31; fr. res. \\
\hline
\texttt{W1p2p2} & u* & 5 & 3000.56 & 25.21 & - & $-2.8 \pm 1.1$ \textbf{(T)}& 0.98 & no ch. 21, 35 \\
\texttt{[w1.$+$2$+$2]} & g' & 5 & 2500.45 & 25.63 & - & $1.4 \pm 1.2$ \textbf{(T)}& 0.95 &  \\
(0.81) & r' & 2 & 1000.18 & 24.53 & - & $-3.4 \pm 0.6$ \textbf{(T)}& 0.95 &  \\
 & i' & 8 & 4960.76 & 24.80 & - & $0.7 \pm 1.1$ \textbf{(T)}& 0.85 &  \\
 & z' & 10 & 6000.95 & 23.73 & - & $-1.1 \pm 1.3$ \textbf{(T)}& 0.74 &  \\
\hline
\texttt{W1p2p3} & u* & 7 & 5950.29 & 25.61 & - & $-0.9 \pm 0.5$ \textbf{(T)}& 1.00 & no ch. 31 \\
\texttt{[w1.$+$2$+$3]} & g' & 5 & 2500.35 & 25.62 & - & $-0.3 \pm 0.5$ \textbf{(T)}& 0.95 &  \\
(0.83) & r' & 4 & 2000.37 & 24.82 & - & $-6.3 \pm 0.9$ \textbf{(T)}& 0.71 &  \\
 & i' & 7 & 4340.55 & 24.59 & - & $-0.4 \pm 0.9$ \textbf{(T)}& 0.95 &  \\
 & z' & 9 & 7200.41 & 23.80 & - & $0.9 \pm 2.3$ \textbf{(T)}& 0.69 & no ch. 31; fr. res. \\
\hline
\texttt{W1p3m0} & u* & 5 & 3000.55 & 25.17 & $11.9 \pm 6.6$ & $6.4 \pm 2.2$ \textbf{(M)}& 0.63 & no ch. 31 \\
\texttt{[w1.$+$3$-$0]} & g' & 5 & 2500.43 & 25.54 & $-1.8 \pm 3.0$ & $-2.6 \pm 0.6$ \textbf{(T)}& 0.87 & no ch. 31; m. ZP \\
(0.81) & r' & 2 & 1000.17 & 24.33 & $2.4 \pm 3.0$ & $0.1 \pm 1.3$ \textbf{(T)}& 0.69 & no ch. 31 \\
 & i' & 5 & 3100.23 & 24.44 & $3.5 \pm 3.5$ & $3.1 \pm 1.0$ \textbf{(T)}& 0.71 & no ch. 31; sat. tr. \\
 & z' & 12 & 7201.49 & 23.59 & $-0.4 \pm 7.2$ & $-8.8 \pm 3.7$ \textbf{(M)}& 0.71 & no ch. 31; fr. res. \\
\hline
\texttt{W1p3p1} & u* & 5 & 3000.26 & 25.31 & - & - & 0.85 & no ch. 31 \\
\texttt{[w1.$+$3$+$1]} & g' & 6 & 3000.27 & 25.62 & - & $0.0 \pm 0.5$ \textbf{(T)}& 0.95 & no ch. 31 \\
(0.85) & r' & 2 & 1000.10 & 24.39 & - & $0.5 \pm 0.7$ \textbf{(T)}& 0.85 & no ch. 31 \\
 & i' & 7 & 4340.32 & 24.60 & - & $-0.8 \pm 1.1$ \textbf{(T)}& 0.95 & no ch. 31 \\
 & z' & 6 & 3600.47 & 23.55 & - & - & 0.69 & no ch. 31 \\
\hline
\texttt{W1p3p2} & u* & 7 & 4200.42 & 25.45 & - & $5.0 \pm 1.5$ \textbf{(M)}& 0.90 & no ch. 31 \\
\texttt{[w1.$+$3$+$2]} & g' & 5 & 2500.41 & 25.54 & - & $0.3 \pm 0.9$ \textbf{(T)}& 0.85 & no ch. 31; m. ZP \\
(0.82) & r' & 3 & 1500.22 & 24.51 & - & $-1.2 \pm 1.2$ \textbf{(T)}& 0.83 & no ch. 31 \\
 & i' & 6 & 3720.24 & 24.48 & - & $0.6 \pm 0.8$ \textbf{(T)}& 0.69 & no ch. 31 \\
 & z' & 6 & 3600.58 & 23.31 & - & $-7.3 \pm 0.9$ \textbf{(M)}& 0.55 & no ch. 31 \\
\hline
\texttt{W1p3p3} & u* & 4 & 2400.39 & 25.01 & - & $3.8 \pm 0.9$ \textbf{(M)}& 1.11 & no ch. 31 \\
\texttt{[w1.$+$3$+$3]} & g' & 5 & 2500.20 & 25.51 & - & $0.1 \pm 0.8$ \textbf{(T)}& 0.95 & no ch. 31 \\
(0.84) & r' & 2 & 1000.10 & 24.39 & - & $-2.9 \pm 0.6$ \textbf{(T)}& 0.87 & no ch. 31 \\
 & i' & 7 & 4340.33 & 24.51 & - & $-1.3 \pm 0.9$ \textbf{(T)}& 0.82 & no ch. 31 \\
 & z' & 6 & 3600.62 & 23.39 & - & $-7.2 \pm 0.9$ \textbf{(M)}& 0.55 & no ch. 31 \\
\hline
\texttt{W1p4m0} & u* & 5 & 3000.54 & 25.35 & $9.4 \pm 4.7$ & $6.4 \pm 0.7$ \textbf{(M)}& 0.72 & no ch. 31 \\
\texttt{[w1.$+$4$-$0]} & g' & 5 & 2500.41 & 25.50 & $-1.5 \pm 3.1$ & $-0.8 \pm 1.1$ \textbf{(T)}& 0.87 & no ch. 31; m. ZP \\
(0.82) & r' & 2 & 1000.19 & 24.33 & $2.7 \pm 2.5$ & $0.3 \pm 0.6$ \textbf{(T)}& 0.71 & no ch. 31 \\
 & i' & 4 & 2480.15 & 24.15 & $0.1 \pm 3.1$ & $0.9 \pm 1.1$ \textbf{(T)}& 0.95 & no ch. 31 \\
 & z' & 6 & 3600.72 & 23.48 & $0.4 \pm 5.9$ & $-7.1 \pm 0.8$ \textbf{(M)}& 0.69 & no ch. 31 \\
\hline
\texttt{W1p4p1} & u* & 5 & 3000.54 & 25.42 & - & - & 0.79 &  \\
\texttt{[w1.$+$4$+$1]} & g' & 5 & 2500.43 & 25.45 & - & $-1.5 \pm 0.7$ \textbf{(T)}& 0.85 & no ch. 31; m. ZP \\
(0.82) & r' & 2 & 1000.16 & 24.21 & - & $1.6 \pm 0.6$ \textbf{(T)}& 0.79 & m. ZP \\
 & i' & 7 & 4340.62 & 24.48 & - & $0.3 \pm 0.8$ \textbf{(T)}& 0.79 & m. ZP \\
 & z' & 6 & 3600.52 & 23.34 & - & - & 0.63 &  \\
\hline
\texttt{W1p4p2} & u* & 5 & 3000.60 & 25.29 & - & - & 0.77 &  \\
\texttt{[w1.$+$4$+$2]} & g' & 5 & 2500.44 & 25.49 & - & $-0.9 \pm 1.3$ \textbf{(T)}& 0.85 & no ch. 31; m. ZP \\
(0.87) & r' & 2 & 1000.16 & 24.22 & - & $-2.2 \pm 0.8$ \textbf{(T)}& 0.74 & m. ZP \\
 & i' & 7 & 4340.64 & 24.44 & - & $-0.9 \pm 1.1$ \textbf{(T)}& 0.87 & m. ZP \\
 & z' & 6 & 3600.50 & 23.45 & - & - & 0.55 &  \\
\hline
\texttt{W1p4p3} & u* & 5 & 3000.25 & 25.32 & - & $5.9 \pm 0.8$ \textbf{(M)}& 0.98 & no ch. 31 \\
\texttt{[w1.$+$4$+$3]} & g' & 5 & 2500.41 & 25.65 & - & $-0.9 \pm 2.3$ \textbf{(T)}& 0.95 & no ch. 31 \\
(0.83) & & & & & & $-1.4 \pm 1.1$ \textbf{(M)} & & \\
 & r' & 2 & 1000.17 & 24.46 & - & $-0.7 \pm 1.0$ \textbf{(T)}& 0.93 & no ch. 31 \\
 & i' & 7 & 4340.34 & 24.44 & - & $-1.0 \pm 0.7$ \textbf{(T)}& 0.95 & no ch. 31 \\
 & z' & 6 & 3600.38 & 23.29 & - & - & 0.77 & no ch. 31 \\
\hline
\hline
\texttt{W3m1m2} & u* & 5 & 3000.96 & 24.78 & $30.2 \pm 3.9$ & $25.9 \pm 2.5$ \textbf{(M)}& 0.87 &  \\
\texttt{[w3.$-$1$-$2]} & g' & 5 & 2501.02 & 25.48 & $0.2 \pm 1.9$ & $0.2 \pm 0.6$ \textbf{(T)}& 0.87 & m. ZP \\
(0.83) & & & & & & $-4.9 \pm 1.5$ \textbf{(M)} & & \\
 & r' & 2 & 1000.47 & 24.51 & $-0.1 \pm 2.7$ & $-1.3 \pm 0.7$ \textbf{(T)}& 0.63 &  \\
 & & & & & & $-9.9 \pm 3.7$ \textbf{(M)} & & \\
 & i' & 7 & 4306.47 & 24.36 & $0.6 \pm 3.8$ & $-0.6 \pm 1.3$ \textbf{(T)}& 0.66 &  \\
 & z' & 6 & 3601.20 & 23.41 & $-6.1 \pm 4.2$ & $-9.4 \pm 2.3$ \textbf{(M)}& 0.67 &  \\
\hline
\texttt{W3m1m3} & u* & 5 & 3000.98 & 24.87 & $29.9 \pm 3.8$ & $26.9 \pm 2.6$ \textbf{(M)}& 0.74 & no ch. 21 \\
\texttt{[w3.$-$1$-$3]} & g' & 5 & 2500.90 & 25.63 & $0.4 \pm 2.0$ & $0.1 \pm 0.5$ \textbf{(T)}& 0.87 & no ch. 21; m. ZP \\
(0.82) & & & & & & $-4.7 \pm 1.1$ \textbf{(M)} & & \\
 & r' & 2 & 1000.28 & 24.52 & $2.9 \pm 2.2$ & $-2.2 \pm 1.6$ \textbf{(M)}& 0.97 & no ch. 21 \\
 & i' & 7 & 4306.61 & 24.36 & $0.6 \pm 2.7$ & $0.3 \pm 0.9$ \textbf{(T)}& 0.66 & no ch. 21; m. ZP \\
 & & & & & & $-4.4 \pm 1.6$ \textbf{(M)} & & \\
 & z' & 6 & 3601.17 & 23.36 & $-3.8 \pm 5.6$ & $-9.1 \pm 2.2$ \textbf{(M)}& 0.59 & no ch. 21 \\
\hline
\texttt{W3m2m2} & u* & 5 & 3001.06 & 25.33 & $29.4 \pm 4.1$ & $25.3 \pm 2.2$ \textbf{(M)}& 0.77 &  \\
\texttt{[w3.$-$2$-$2]} & g' & 5 & 2500.89 & 25.59 & $0.7 \pm 2.2$ & $-0.3 \pm 0.5$ \textbf{(T)}& 0.90 &  \\
(0.85) & & & & & & $-3.8 \pm 1.0$ \textbf{(M)} & & \\
 & r' & 2 & 1000.42 & 24.56 & $0.7 \pm 2.7$ & $-1.1 \pm 1.0$ \textbf{(T)}& 0.57 &  \\
 & & & & & & $-4.8 \pm 2.2$ \textbf{(M)} & & \\
 & i' & 7 & 4306.23 & 24.46 & $0.3 \pm 2.7$ & $0.2 \pm 0.8$ \textbf{(T)}& 0.66 &  \\
 & z' & 6 & 3601.22 & 23.43 & $-3.3 \pm 4.9$ & $-8.5 \pm 1.7$ \textbf{(M)}& 0.64 &  \\
\hline
\texttt{W3m3m2} & u* & 5 & 3000.99 & 25.27 & $29.0 \pm 5.0$ & - & 0.68 &  \\
\texttt{[w3.$-$3$-$2]} & g' & 5 & 2500.87 & 25.40 & $0.4 \pm 2.2$ & $-0.2 \pm 1.1$ \textbf{(T)}& 0.66 &  \\
(0.84) & r' & 2 & 1000.40 & 24.20 & $4.5 \pm 2.4$ & $1.9 \pm 0.7$ \textbf{(T)}& 0.66 &  \\
 & i' & 7 & 4306.27 & 24.43 & $0.1 \pm 3.3$ & $0.0 \pm 0.9$ \textbf{(T)}& 0.53 &  \\
 & z' & 6 & 3601.20 & 23.30 & $-2.3 \pm 4.7$ & - & 0.55 &  \\
\hline
\texttt{W3m3m3} & u* & 5 & 3001.02 & 25.29 & $28.8 \pm 4.1$ & - & 0.74 &  \\
\texttt{[w3.$-$3$-$3]} & g' & 5 & 2500.93 & 25.52 & $0.2 \pm 2.3$ & $-0.5 \pm 0.6$ \textbf{(T)}& 0.82 &  \\
(0.83) & r' & 2 & 1000.42 & 24.25 & $4.4 \pm 2.6$ & $1.4 \pm 0.6$ \textbf{(T)}& 0.66 &  \\
 & i' & 7 & 4306.19 & 24.49 & $-0.8 \pm 3.0$ & $0.1 \pm 0.8$ \textbf{(T)}& 0.50 &  \\
 & z' & 6 & 3601.21 & 23.49 & $-3.1 \pm 5.5$ & - & 0.58 &  \\
\hline
\hline
\texttt{W4m0m0} & u* & 5 & 3000.26 & 25.38 & $26.4 \pm 3.8$ & - & 1.03 &  \\
\texttt{[w4.$+$0$+$0]} & g' & 5 & 2500.40 & 25.43 & $-0.1 \pm 2.0$ & $-1.9 \pm 0.6$ \textbf{(M)}& 0.79 &  \\
(0.82) & r' & 3 & 1500.22 & 24.23 & $-0.2 \pm 2.2$ & $1.0 \pm 0.6$ \textbf{(M)}& 0.61 &  \\
 & i' & 7 & 4305.65 & 24.62 & $5.3 \pm 3.3$ & - & 0.71 &  \\
 & z' & 12 & 7200.87 & 23.78 & $-2.3 \pm 4.6$ & - & 0.66 &  \\
\hline
\texttt{W4m0m1} & u* & 5 & 3000.29 & 25.30 & $23.2 \pm 4.0$ & - & 0.74 &  \\
\texttt{[w4.$+$0$-$1]} & g' & 10 & 5000.68 & 25.85 & $-0.2 \pm 2.5$ & $-7.7 \pm 1.6$ \textbf{(M)}& 0.82 &  \\
(0.83) & r' & 2 & 1000.10 & 24.30 & $1.7 \pm 2.3$ & $-5.4 \pm 1.7$ \textbf{(M)}& 0.67 &  \\
 & i' & 7 & 4305.36 & 24.62 & $-0.8 \pm 3.0$ & - & 0.56 &  \\
 & z' & 6 & 3600.27 & 23.29 & $-3.2 \pm 5.0$ & - & 0.50 &  \\
\hline
\texttt{W4m0m2} & u* & 5 & 3000.31 & 25.41 & $24.0 \pm 4.5$ & - & 0.71 &  \\
\texttt{[w4.$+$0$-$2]} & g' & 10 & 5000.58 & 25.83 & $-0.3 \pm 1.9$ & $-6.2 \pm 1.2$ \textbf{(M)}& 0.77 &  \\
(0.81) & r' & 2 & 1000.10 & 24.28 & $2.1 \pm 2.2$ & - & 0.58 &  \\
 & i' & 7 & 4305.58 & 24.77 & $0.7 \pm 2.6$ & - & 0.61 &  \\
 & z' & 6 & 3600.34 & 23.62 & $-4.4 \pm 4.1$ & - & 0.63 &  \\
\hline
\texttt{W4m1m1} & u* & 5 & 3000.24 & 25.26 & $24.2 \pm 3.9$ & - & 0.69 &  \\
\texttt{[w4.$-$1$-$1]} & g' & 13 & 6500.96 & 26.00 & $2.9 \pm 2.4$ & - & 0.79 &  \\
(0.79) & r' & 2 & 1000.16 & 24.32 & $1.4 \pm 2.5$ & - & 0.87 &  \\
 & i' & 6 & 3690.44 & 24.62 & $-0.2 \pm 3.2$ & - & 0.71 &  \\
 & z' & 5 & 3000.24 & 23.28 & $-1.2 \pm 4.8$ & - & 0.48 &  \\
\hline
\texttt{W4m1m2} & u* & 6 & 3600.41 & 25.45 & $33.2 \pm 8.1$ & - & 0.66 &  \\
\texttt{[w4.$-$1$-$2]} & g' & 5 & 2500.53 & 25.54 & $-1.8 \pm 1.8$ & $-7.6 \pm 1.3$ \textbf{(M)}& 0.79 &  \\
(0.82) & r' & 2 & 1000.15 & 24.34 & $2.9 \pm 2.4$ & - & 0.50 &  \\
 & i' & 7 & 4305.43 & 24.60 & $1.8 \pm 2.9$ & - & 0.72 &  \\
 & z' & 5 & 3000.38 & 23.37 & $-0.3 \pm 4.7$ & - & 0.51 &  \\
\hline
\texttt{W4p1m0} & u* & 5 & 3000.43 & 25.29 & $26.2 \pm 4.1$ & - & 0.90 &  \\
\texttt{[w4.$+$1$+$0]} & g' & 5 & 2500.30 & 25.40 & $1.6 \pm 2.1$ & $-2.3 \pm 0.6$ \textbf{(M)}& 0.67 &  \\
(0.75) & r' & 2 & 1000.16 & 24.35 & $3.0 \pm 2.2$ & - & 0.94 &  \\
 & i' & 7 & 4305.52 & 24.31 & $0.4 \pm 3.3$ & - & 0.53 &  \\
 & z' & 6 & 3600.36 & 23.33 & $-5.0 \pm 4.2$ & - & 0.55 &  \\
\hline
\texttt{W4p1m1} & u* & 5 & 3000.22 & 25.33 & $27.5 \pm 3.8$ & - & 0.85 &  \\
\texttt{[w4.$+$1$-$1]} & g' & 5 & 2500.34 & 25.33 & $1.2 \pm 2.0$ & - & 0.83 &  \\
(0.80) & r' & 2 & 1000.17 & 24.28 & $-0.8 \pm 2.5$ & - & 0.67 &  \\
 & i' & 14 & 8611.03 & 24.86 & $1.4 \pm 3.7$ & - & 0.66 &  \\
 & z' & 6 & 3600.33 & 23.35 & $-4.2 \pm 4.7$ & - & 0.63 &  \\
\hline
\texttt{W4p1m2} & u* & 5 & 3000.39 & 25.15 & $12.7 \pm 3.9$ & - & 0.87 &  \\
\texttt{[w4.$+$1$-$2]} & g' & 5 & 2500.31 & 25.37 & $0.9 \pm 1.9$ & $-4.9 \pm 1.3$ \textbf{(M)}& 0.85 &  \\
(0.82) & r' & 2 & 1000.10 & 24.34 & $1.7 \pm 2.1$ & - & 0.61 &  \\
 & i' & 7 & 4305.41 & 24.57 & $1.1 \pm 3.4$ & $-5.8 \pm 1.1$ \textbf{(M)}& 0.71 &  \\
 & z' & 5 & 3000.48 & 23.12 & $-2.1 \pm 5.0$ & - & 0.53 &  \\
\hline
\texttt{W4p2m0} & u* & 5 & 3000.31 & 25.24 & $28.2 \pm 4.4$ & - & 0.79 &  \\
\texttt{[w4.$+$2$-$0]} & g' & 5 & 2500.47 & 25.30 & $-1.6 \pm 2.4$ & $-4.4 \pm 1.6$ \textbf{(M)}& 0.74 &  \\
(0.77) & r' & 2 & 1000.14 & 24.36 & $2.0 \pm 2.3$ & - & 0.63 &  \\
 & i' & 7 & 4305.53 & 24.68 & $0.0 \pm 3.0$ & - & 0.57 &  \\
 & z' & 6 & 3600.39 & 23.20 & $-4.9 \pm 3.9$ & - & 0.79 &  \\
\hline
\texttt{W4p2m1} & u* & 5 & 3000.36 & 25.18 & $19.7 \pm 3.7$ & $14.5 \pm 2.0$ \textbf{(M)}& 0.98 &  \\
\texttt{[w4.$+$2$-$1]} & g' & 5 & 2500.39 & 25.45 & $-0.7 \pm 1.9$ & $-6.4 \pm 1.1$ \textbf{(M)}& 0.85 &  \\
(0.80) & r' & 2 & 1000.22 & 24.12 & $1.6 \pm 2.4$ & - & 0.85 &  \\
 & i' & 7 & 4305.69 & 24.53 & $-3.4 \pm 2.9$ & $-9.9 \pm 0.9$ \textbf{(M)}& 0.66 &  \\
 & z' & 12 & 7200.72 & 23.77 & $-8.0 \pm 4.5$ & $-15.7 \pm 2.1$ \textbf{(M)}& 0.74 &  \\
\hline
\texttt{W4p2m2} & u* & 4 & 2400.24 & 25.18 & $16.4 \pm 3.7$ & - & 1.00 &  \\
\texttt{[w4.$+$2$-$2]} & g' & 5 & 2500.37 & 25.36 & $-1.3 \pm 2.1$ & - & 0.77 &  \\
(0.83) & r' & 2 & 1000.22 & 24.05 & $2.5 \pm 2.5$ & - & 0.90 &  \\
 & i' & 13 & 7995.87 & 24.98 & $1.9 \pm 4.1$ & - & 0.63 &  \\
 & z' & 10 & 6000.55 & 23.66 & $-3.7 \pm 4.0$ & - & 0.72 &  \\
\hline
\hline
\end{longtable}

